Fairness Reprogramming

Despite a surge of recent advances in promoting machine Learning (ML) fairness, the existing mainstream approaches mostly require retraining or finetuning the entire weights of the neural network to meet the fairness criteria. However, this is often infeasible in practice for those large-scale trained models due to large computational and storage costs, low data efficiency, and model privacy issues. In this paper, we propose a new generic fairness learning paradigm, called FairReprogram, which incorporates the model reprogramming technique. Specifically, FairReprogram considers the case where models can not be changed and appends to the input a set of perturbations, called the fairness trigger, which is tuned towards the fairness criteria under a min-max formulation. We further introduce an information-theoretic framework that explains why and under what conditions fairness goals can be achieved using the fairness trigger. We show both theoretically and empirically that the fairness trigger can effectively obscure demographic biases in the output prediction of fixed ML models by providing false demographic information that hinders the model from utilizing the correct demographic information to make the prediction. Extensive experiments on both NLP and CV datasets demonstrate that our method can achieve better fairness improvements than retraining-based methods with far less data dependency under two widely-used fairness criteria. Codes are available at https://github.com/UCSB-NLP-Chang/Fairness-Reprogramming.git.

==> ArXiv Fairness Reprogramming/analysis.tex <==
\begin{table*}[t]
	\small
	\begin{tabular}{p{0.77\textwidth}c}
        \emph{Text (Non-toxic)} & \emph{Predicted Toxicity} \\
		\arrayrulecolor{grey}  
		\midrule
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlg{\ul{\textbf{the}}}{15} \hlr{\ul{\textbf{mirror}}}{20} & 0.149 \\
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlr{the}{0} \hlr{mirror}{0} \,\,\,\,
        \hlr{same}{0} \hlr{\ul{\textbf{diocesan}}}{15} \hlg{\ul{\textbf{bula}}}{20} \hlr{\ul{\textbf{rev}}}{8} \hlr{\ul{\textbf{proceedings}}}{8} & 0.069 \\
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlr{the}{0} \hlr{mirror}{0}  \,\,\,\,
        \hlr{soto}{0} \hlr{\ul{\textbf{cc}}}{10} \hlr{rib}{0} \hlr{\ul{\textbf{hebrew}}}{10} \hlr{armenian}{0} & 0.054 \\
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlr{the}{0} \hlg{\ul{mirror}}{0}  \,\,\,\,
        \hlr{\ul{\textbf{paul}}}{10} \hlr{long}{0} \hlr{course}{0} \hlr{\ul{\textbf{parish}}}{10} \hlr{\ul{\textbf{body}}}{10} & 0.073 \\
	\end{tabular}
    \captionof{figure}{\small{
    A text example from \texttt{Civil Comments} with \textsc{Integrated Gradient}~\cite{Sundararajan2017AxiomaticAF,kokhlikyan2020captum}  highlighting important words that influence \textsc{ERM} model predictions.
    The text is concatenated with three triggers generated with different adversary weight.
    \hlg{\ul{\textbf{Green highlights}}}{20} the words that lean to toxic predictions and 
    \hlr{\ul{\textbf{Red highlights}}}{20} non-toxic leaning words.
    The model prediction tends to be correct after adding the triggers.
    }}
    \label{fig: vis_nlp}
    \vspace*{-4mm}
\end{table*}

\begin{wrapfigure}{r}{80mm}
    \vspace*{-4mm}
    \centering
    \includegraphics[width=\linewidth]{figures/grad_cam_small.png}
    \vspace*{-4.5mm}
    \caption{\footnotesize{Gradient-based saliency map visualized with \textsc{Grad Cam}~\cite{selvaraju2017grad} of different methods. 
    The highlighted zones (marked in red) depicting regions exerting major influence on the predicted labels (non-blond hair v.s. blond hair) in each row, which also depict the attention of the model on the input image.
    }}
    \label{fig: vis_cv}
    \vspace*{-1mm}
\end{wrapfigure}

\vspace*{-0.1in}
\paragraph{Input saliency attribution.}
Fig.~\ref{fig: vis_nlp} and \ref{fig: vis_cv} compare the saliency maps of some example inputs with and without the fairness triggers. Specifically, 
For the NLP applications, we extract a subset of \texttt{Civil Comments} with religion-related demographic annotations,
and apply IG~\cite{Sundararajan2017AxiomaticAF} to localize word pieces that contribute most to the text toxicity classification.  For the CV application, we use GradCam~\cite{selvaraju2017grad} to identify class-discriminative regions of   {\texttt{CelebA}}'s  test images.
As shown in Fig.~\ref{fig: vis_nlp}, our fairness trigger consists of a lot of religion-related words (\textit{e.g.}, diocesan, hebrew, parish). Meanwhile, the predicted toxicity score of the benign text starting from `muslims' significantly reduces. These observations verify our theoretical hypothesis that the fairness trigger is strongly indicative of a certain demographic group to prevent the classifier from using the true demographic information.
In addition, Fig.~\ref{fig: vis_cv} presents the input saliency maps on two input images with respect to their predicted labels, non-blond hair and blond hair, respectively. As can be observed, when there is no fairness trigger, the saliency region incorrectly concentrates on the facial parts, indicating the classifier is likely to use biased information, such as gender, for its decision. With the fairness trigger, the saliency region moves to the hair parts, which matches the behavior of \textsc{AdvIn}. These results confirm that our fairness trigger can drive models to make fairer predictions.



==> ArXiv Fairness Reprogramming/exp.tex <==
\section{Experiments}
In this section, we evaluate the effectiveness of {\ours} on both NLP and CV applications in terms of accuracy, fairness, performances under low-data regime, transferability and interpretability.

\subsection{Experiment Setup}
\label{sec: setup}
\paragraph{Datasets}We consider the following two commonly used  NLP and CV datasets:
\begin{itemize}[leftmargin=9pt,topsep=0pt]
    \vspace{-1mm}
    \item
    \texttt{\textbf{Civil Comments}}~\cite{Koh2021WILDSAB,AI2019JigsawUB}:
    The dataset contains 448k texts with labels that depict the toxicity of each input. The demographic information of each text is provided.  
    \vspace{-1mm}
    
    \item 
    \textbf{\texttt{CelebA}}~\cite{liu2015faceattributes}: 
    The dataset contains over 200k human face images and each contains 39 binary attribute annotations.  We follow the conventional setting \cite{liu2015faceattributes} that adopts the hair color prediction task in our experiment and uses gender annotation as the demographic information.\,\cite{xu2020investigating, dash2020counterfactual, hwang2020fairfacegan}   
    \vspace{-1mm}
\end{itemize}

For both datasets, we split the entire data into a training set, a tuning set, a validation set, and a testing set.  The training set is used for the base model training, \emph{i.e.}, to obtain a biased model for reprogramming.  The tunning set and validation set are used for trigger training and hyper-parameter selection.  We report our results on the testing set.   It is worth mentioning that there is no overlapping data between different sets and the size of the tuning set is much smaller than the training one.  Specifically, we set the size ratio between the tunning set and the training as $1/5$ and $1/100$ for \texttt{Civil Comments} and \texttt{CelebA}, respectively.  
The full statistics of the datasets can be found in Appendix~\ref{app: data_statistic}.

\paragraph{Metrics} Besides the model accuracy, we introduce two empirical fairness metrics, one under each of the two fairness criteria as in Eq.~\eqref{eq:fair_criteria}. For binary classification, the metrics are calculated as:
\begin{equation*}
    % \small
    \mbox{\textbf{DP:}}\sum_{z\in \mathcal{Z}} |\text{p}(\hat{Y}=1)-\text{p}(\hat{Y}=1|Z=z)|, \quad \mbox{\textbf{EO:}} \sum_{z\in \mathcal{Z}} (|\text{FPR}-\text{FPR}_z| + |\text{FNR} - \text{FNR}_z|)/2,
\end{equation*}
where DP and EO stand for demographic parity and equalized odds respectively. $\text{FPR}$ and $\text{FNR}$ are the false positive/negative rate, and the subscript $z$ denotes the score is calculated within a specific demographic group $Z=z$.  For example, $\text{FPR}_{male}$ indicates the false positive rate calculated over all examples with the ``male'' annotation. For a multi-class setting, the bias scores are first calculated similarly using one-vs-all for each class and then averaged across different classes.  
All reported results are the average of three different random runs.  
It can be shown that these metrics are non-negative, and will become zero when their corresponding fairness criteria are achieved.
For better elaboration, we report the negative bias scores in our experiments,
so the larger these negative scores are, 
the better the model satisfies the corresponding fairness criteria. 


\paragraph{Baselines and implementation details}
We consider the following models for comparison:

$\bullet$ \textsc{Base}: the base model to be reprogrammed, trained with the cross-entropy loss on the training set.  

$\bullet$ {\adv}~\cite{Zhang2018MitigatingUB}: an in-processing adversarial training method that optimizes both model accuracy and fairness using the training set.  

$\bullet$ {\advp}: a post-processing variant of {\adv}, which fine-tunes the \textsc{Base} model with the same fairness-aware adversarial objectives as {\adv}, but using the (low-resource) tunning set only.  

For NLP experiments, we use a pre-trained \textsc{Bert} \cite{Devlin2019BERTPO} to obtain the \textsc{Base} and {\adv} models.  We use \textsc{AdamW} \cite{loshchilov2017decoupled} as the optimizer, and set the learning rate to $10^{-5}$ for all baselines and $0.1$ for {\ours}.  For CV experiments, we consider a \textsc{ResNet-18} \cite{he2016deep} that pre-trained on ImageNet.  
The discriminator used in {\adv}, {\advp} and {\ours} is a three-layer MLP, and the parameters are optimized using \textsc{Adam} with a learning rate of $0.01$.  We pick the best model based on the accuracy (for the \textsc{Base}) or the bias scores (for all other debiasing methods) of the validation set.  \CR{We refer to Appendix~\ref{app: training_detail} for more details and Appendix\,\ref{app: additional_results} for more baseline studies.}

Next we introduce the implementation details of the triggers for different variants of {\ours}. For image classification task, we adopt the border and patch trigger as shown in Fig.\,\ref{fig: trigger}, termed \textsc{FairReprogram (Border)} and \textsc{FairReprogram (Patch)} correspondingly. We define the trigger size as the width of the trigger frame for border trigger and the width of the square patch for patch trigger. Unless otherwise stated, the default trigger size for each setting are $20$ and $80$. 

For text classification task, we introduce a probability vector $\bm v_i 
$ to control the selection of trigger word for each position $i$. 
Specifically, we have the trigger $\bm \delta_i = \bm E \bm v_i$ where $\bm E 
$ represents the pretrained word embedding matrix of \textsc{Bert}.
Then we simply concatenate $\bm \delta$ after all input texts\footnote{The trigger is appended as a suffix after all input tokens but before [SEP] for \textsc{Bert}.} in the embeddings space as the fairness trigger. We introduce two types of trigger. The first type, called \textsc{FairReprogram (Soft)} , uses continuous \e{\bm v_i}'s, and each  \e{\bm v_i} is projected onto the continuous probability simplex using the bisection algorithm after each training step. The second type, called \textsc{FairReprogram (Hard)}, discretizes each $\bm v_i$ into a one-hot vector $\hat{\bm v}_i$ via $\mathop{\arg\max}$ operation.  
We adopt the straight through technique~\cite{Bengio2013EstimatingOP} to update $\bm v_i$ during training.
The triggers found by \textsc{FairReprogram (Hard)} enjoy better interpretability as they correspond to a sequence of word tokens.
Unless specified otherwise, we set the trigger word number as five for our experiments.


\subsection{Results}


\begin{figure}[!t]
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figures/gh_figures/ED_PO1_AcrossZ.pdf} &
    \hspace*{-4mm}  \includegraphics[width=.25\textwidth,height=!]{figures/gh_figures/ED_FR_AcrossZ.pdf} &
    \hspace*{-4mm}  \includegraphics[width=.25\textwidth,height=!]{figures/2class.pdf} &
    \hspace*{-4mm} \includegraphics[width=.25\textwidth,height=!]{figures/2class_y.pdf} \\
    \multicolumn{2}{c}{\footnotesize{(a) \texttt{Civil Comments}}} & \multicolumn{2}{c}{\footnotesize{(b) \texttt{CelebA}}}
\end{tabular}}
\caption{\footnotesize{Results on (a) \texttt{Civil Comments} and (b) \texttt{CelebA}. We report the negative DP (left) and the negative EO (right) scores.  For each method, we vary the trade-off parameter $\lambda$ (as shown in \eqref{eq:loss}) to record the performance.  The closer a dot to the upper-right corner, the better the model is.   We consider five different $\lambda$s for each method. 
The solid curve is the fitted polynomial with order 30. 
}}
\label{fig: exp_overview}
\end{figure}


\begin{figure}[!t]
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figures/gh_figures/ED_PO1_AcrossZ_data_size.pdf} &
    \hspace*{-4mm}  \includegraphics[width=.25\textwidth,height=!]{figures/gh_figures/ED_FR_AcrossZ_data_size.pdf} &
    \hspace*{-4mm}  \includegraphics[width=.25\textwidth,height=!]{figures/few-n.pdf} &
    \hspace*{-4mm} \includegraphics[width=.25\textwidth,height=!]{figures/few-y.pdf} \\
    \multicolumn{2}{c}{\footnotesize{(a) \texttt{Civil Comments}}} & \multicolumn{2}{c}{\footnotesize{(b) \texttt{CelebA}}}
\end{tabular}}
\caption{\footnotesize{
Results on (a) \texttt{Civil Comments} and (b) \texttt{CelebA} with different tuning data ratio. We report the negative DP (left) and negative EO (right) scores.
We consider a fixed \textsc{Base} model trained with training set, whose negative bias scores are presented as a black dashed line.
Then we train other methods with different tuning data ratio to promote fairness of the \textsc{Base} model.
}}
% \vspace*{-0.1in}
\label{fig: limit_data}
\end{figure}
Fig.~\ref{fig: exp_overview} shows the performance of the proposed \textsc{FairReprogram} with other baselines on both NLP (subfigure (a)) and CV (subfigure (b)) datasets using DP (left) and EO (right) metrics. In each subfigure, the data samples of the same method (dots in the same color) are generated by explicit changing the adversary weight $\lambda$ in \eqref{eq:loss}, which controls the trade-off between fairness and accuracy. We further fit the data with polynomial regression to present the curves. Appendix\,\ref{app: training_detail} shows the detailed $\lambda$ choices for different methods.
Here are our key observations.  \underline{{First}}, our method improves the fairness of the \textsc{Base} model.  In particular, our methods (both \textcolor{orange}{orange} and \textcolor{red}{red} curves) achieve higher negative DP and EO scores with a comparable classification accuracy.    \underline{Second}, our method enjoys a better fairness-accuracy trade-off compared with all other baselines.  Specifically, the curves of our method lie farther to the upper-right corner of the plots, which implies that our method improves model fairness with fewer sacrifices on accuracy.   It is also worth noting that although {\adv} achieves good fairness scores, it uses much more data for training.  




\paragraph{Limited data setting} 
We further evaluate {\advp} and {\ours} with decreasing the number of data in the tuning set.
Specifically, we fix a $\lambda$ for each method such that all methods  achieve comparable bias score with full tuning set.
The detailed $\lambda$ choices are provided in Appendix~\ref{app: training_detail}.
Then we apply these methods to subsets of the tuning set with different proportions.
The results are shown in Fig.~\ref{fig: limit_data}. There are two key observations.
\underline{First}, our method can consistently improve fairness upon \textsc{Base} model even with 1\% tuning data, indicating a high data efficiency of {\ours}.
\underline{Second}, {\ours} achieves better fairness than {\advp} does when tuning data number decreases.
For example, in Fig.~\ref{fig: limit_data} (a), the curve of our method is significantly above the {\advp} as tuning data decreases.
When the tuning set size is extremely small, {\advp} significantly deteriorates and even underperforms the \textsc{Base} model.

\paragraph{Transferability} 
\begin{figure}[!t]
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figures/gh_figures/ED_PO1_AcrossZ-transfer.pdf} &
    \hspace*{-4mm}  \includegraphics[width=.25\textwidth,height=!]{figures/gh_figures/ED_FR_AcrossZ-transfer.pdf} &
    \hspace*{-4mm}  \includegraphics[width=.25\textwidth,height=!]{figures/transfer.pdf} &
    \hspace*{-4mm} \includegraphics[width=.25\textwidth,height=!]{figures/transfer_y.pdf} \\
    \multicolumn{2}{c}{\footnotesize{(a) \texttt{Civil Comments}}} & \multicolumn{2}{c}{\footnotesize{(b) \texttt{CelebA}}}
\end{tabular}}
\caption{\footnotesize{ 
Results 
in the transfer setting. We report negative DP (left) and negative EO (right) scores. 
The triggers are firstly trained in a \textsc{Base} model.
Then we evaluate the triggers based on another unseen \textsc{Base} model.
We change the parameter $\lambda$ to trade-off accuracy with fairness and draw the curves in the same way with Fig.~\ref{fig: exp_overview}.
The \FiveStar\,  point corresponds to the average of all \textsc{Base} models with different random seeds.
}}
% \vspace*{-4mm}
\label{fig: transfer}
\end{figure}

\begin{wrapfigure}{r}{80mm}
    \vspace*{-6mm}
    \centering
    \includegraphics[width=\linewidth]{figures/grad_cam_small.png}
    \vspace*{-4.5mm}
    \caption{\footnotesize{Gradient-based saliency map visualized with \textsc{Grad Cam}~\cite{selvaraju2017grad} of different methods. 
    The highlighted zones (marked in red) depicting regions exerting major influence on the predicted labels (non-blond hair v.s. blond hair) in each row, which also depict the attention of the model on the input image.
    }}
    \label{fig: vis_cv}
    \vspace*{-4mm}
\end{wrapfigure}

Next, we show the transferability of the fairness triggers found by {\ours}.
We first tune the triggers with a \textsc{Base} source model and then apply the trigger on a target model trained with a different random seed.
The results are shown in Fig.~\ref{fig: transfer}.
As can be seen, {\ours} achieves comparable fairness-accuracy trigger on both the source model and the target model, indicating our method has a good transferability.
This intriguing property brings two benefits of our method: 
\ding{172} if ML model parameters are infeasible (\emph{e.g.} when ML models are provided as services), the users could train a surrogate model and tune the trigger based on it to promote fairness of the original model; 
\ding{173} when ML model parameters are updated with new data (\emph{e.g.} online learning), the user could still use the original trigger for fixing fairness problems.
We further elaborate the results of {\ours} for transferring to different tasks and model architectures in Appendix~\ref{app:transfer}.

\paragraph{Input saliency attribution.}
Fig.~\ref{fig: vis_nlp} and \ref{fig: vis_cv} compare the saliency maps of some example inputs with and without the fairness triggers. Specifically, 
For the NLP applications, we extract a subset of \texttt{Civil Comments} with religion-related demographic annotations,
and apply IG~\cite{Sundararajan2017AxiomaticAF} to localize word pieces that contribute most to the text toxicity classification.  For the CV application, we use GradCam~\cite{selvaraju2017grad} to identify class-discriminative regions of {\texttt{CelebA}}'s  test images.
As shown in Fig.~\ref{fig: vis_nlp}, our fairness trigger consists of a lot of religion-related words (\textit{e.g.}, diocesan, hebrew, parish). Meanwhile, the predicted toxicity score of the benign text starting from `muslims' significantly reduces. These observations verify our theoretical hypothesis that the fairness trigger is strongly indicative of a certain demographic group to prevent the classifier from using the true demographic information.
In addition, Fig.~\ref{fig: vis_cv} presents the input saliency maps on two input images with respect to their predicted labels, non-blond hair and blond hair, respectively. As can be observed, when there is no fairness trigger, the saliency region incorrectly concentrates on the facial parts, indicating the classifier is likely to use biased information, such as gender, for its decision. With the fairness trigger, the saliency region moves to the hair parts, which matches the behavior of \textsc{AdvIn}. These results confirm that our fairness trigger can drive models to make fairer predictions.

\begin{wraptable}{r}{0.5\textwidth}
\vspace*{-4mm}
\centering
\caption{\footnotesize{Predictions of the demographic classifier on a null input with triggers generated by different $\lambda$. The demographic prediction for CV triggers indicate the predicted score for \emph{Male} and \emph{Female}, and it is \emph{Christian}, \emph{Muslim} and \emph{Other religion} for NLP.
}}
\label{tab: demo_classifier}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{cc}
\toprule[1pt]
\midrule
Trigger & Demographic Prediction\\
\midrule
\includegraphics[width=0.05\textwidth]{figures/trigger1.png} & 0.85, 0.15\\
\includegraphics[width=0.05\textwidth]{figures/trigger2.png} & 0.92, 0.08\\
\includegraphics[width=0.05\textwidth]{figures/trigger3.png} & 0.80, 0.20\\
\midrule
same diocesan bula rev proceedings & 0.96, 0.11, 0.02 \\
soto cc rib hebrew armenian & 0.51, 0.08, 0.81 \\
paul long course parish body & 0.98, 0.04, 0.03 \\
\midrule
\bottomrule[1pt]
\end{tabular}}
% \vspace*{-4mm}
\end{wraptable}

\begin{table*}[t]
	\small
	\begin{tabular}{p{0.77\textwidth}c}
        \emph{Text (Non-toxic)} & \emph{Predicted Toxicity} \\
		\arrayrulecolor{grey}  
		\midrule
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlg{\ul{\textbf{the}}}{15} \hlr{\ul{\textbf{mirror}}}{20} & 0.149 \\
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlr{the}{0} \hlr{mirror}{0} \,\,\,\,
        \hlr{same}{0} \hlr{\ul{\textbf{diocesan}}}{15} \hlg{\ul{\textbf{bula}}}{20} \hlr{\ul{\textbf{rev}}}{8} \hlr{\ul{\textbf{proceedings}}}{8} & 0.069 \\
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlr{the}{0} \hlr{mirror}{0}  \,\,\,\,
        \hlr{soto}{0} \hlr{\ul{\textbf{cc}}}{10} \hlr{rib}{0} \hlr{\ul{\textbf{hebrew}}}{10} \hlr{armenian}{0} & 0.054 \\
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlr{the}{0} \hlg{\ul{mirror}}{0}  \,\,\,\,
        \hlr{\ul{\textbf{paul}}}{10} \hlr{long}{0} \hlr{course}{0} \hlr{\ul{\textbf{parish}}}{10} \hlr{\ul{\textbf{body}}}{10} & 0.073 \\
	\end{tabular}
    \captionof{figure}{\small{
    A text example from \texttt{Civil Comments} with \textsc{Integrated Gradient}~\cite{Sundararajan2017AxiomaticAF,kokhlikyan2020captum}  highlighting important words that influence \textsc{ERM} model predictions.
    The text is concatenated with three triggers generated with different adversary weight.
    \hlg{\ul{\textbf{Green highlights}}}{20} the words that lean to toxic predictions and 
    \hlr{\ul{\textbf{Red highlights}}}{20} non-toxic leaning words.
    The model prediction tends to be correct after adding the triggers.
    }}
    \label{fig: vis_nlp}
\end{table*}

To further verify that the triggers encode demographic information, we trained a demographic classifier to predict the demographics from the input (texts or images) without triggers.
The obtained demographic classifiers can accurately identify the demographics contained in the inputs and achieve over 0.99 AUC for identifying demographics in the validation datasets.
Then, we use the demographic classifier to predict the demographic information of a null image/text\footnote{We use an empty string as the null text and an all-black image as the null image.} with the trigger.
Specifically, we select three triggers generated with different $\lambda$ values for both two datasets.
The results\footnote{One text could contain multiple religions so the probabilities do not sum to one for NLP triggers.} can be seen in Table~\ref{tab: demo_classifier}.
We see that the demographic classifier gives confident outputs on the triggers. 
For example, we see that the trigger \emph{paul long course parish body} is classified as containing \emph{christian} with 0.98 confidence, indicating that the found triggers are highly indicative of demographics.
This is consistent with our perspective in Section~\ref{sec:perspective} that the fairness triggers are encoding fake demographic information to obscure ML models from making biased predictions.


\subsection{Multi-Class Classification}

\begin{figure}[!t]
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figures/multi-3-n.pdf} &
    \hspace*{-4mm}  \includegraphics[width=.25\textwidth,height=!]{figures/multi-3-y.pdf} &
    \hspace*{-4mm}  \includegraphics[width=.25\textwidth,height=!]{figures/multi-4-n.pdf} &
    \hspace*{-4mm} \includegraphics[width=.25\textwidth,height=!]{figures/multi-4-y.pdf} \\
    \footnotesize{(a) 8-class negative DP} &   \footnotesize{(b) 8-class negative EO} & \footnotesize{(c) 16-class negative DP} &   \footnotesize{(d) 16-class negative EO}
\end{tabular}}
\caption{\footnotesize{Performance of multi-class classification.  For (a) and (b), we use the attributes \textit{Blond Hair, Smiling, Attractive} for multi-class construction.  We add an addition attribute \textit{Wavy Hair} for (c) and (d).}}
% \vspace*{-5mm}
\label{fig: multi-class}
\end{figure}
To extend our evaluation to a multi-class setting,  we use the \texttt{CelebA} dataset and select $n$ binary attributes that may be spuriously correlated with \emph{gender} \cite{xu2020investigating, dash2020counterfactual, hwang2020fairfacegan}.    Then, following \cite{zhuang2018multi}, we construct data groups by enumerating all $2^n$ possible binary vectors, where each dimension corresponds to a binary attribute.  We index these vectors and treat them as the class labels.  Fig.~\ref{fig: multi-class} shows the accuracy-fairness trade-off curves similar to Fig.~\ref{fig: exp_overview}. It can be observed that our method outperforms the other methods as the \textcolor{red}{red} curves are closer to the top-right corner.   Also, as the class label number increases, the post-processing-based {\advp} falls behind its in-processing counterpart {\adv}, indicating a larger class number may induce more challenges to post-processing methods. 


\subsection{Ablation Studies}
\label{sec: ablation_study}

\begin{figure}[!t]
\centerline{
\begin{tabular}{cccc}
    \hspace*{-2mm} \includegraphics[width=.25\textwidth,height=!]{figures/gh_figures/ED_PO1_AcrossZ_trigger_size.pdf} &
    \hspace*{-4mm}  \includegraphics[width=.25\textwidth,height=!]{figures/gh_figures/ED_FR_AcrossZ_trigger_size.pdf} &
    \hspace*{-4mm}  \includegraphics[width=.25\textwidth,height=!]{figures/trigger_border.pdf} &
    \hspace*{-4mm} \includegraphics[width=.25\textwidth,height=!]{figures/trigger_patch.pdf} \\
    \multicolumn{2}{c}{\footnotesize{(a) \texttt{Civil Comments}}} & \multicolumn{2}{c}{\footnotesize{(b) \texttt{CelebA}}}
\end{tabular}}
\vspace*{-1mm}
\caption{\footnotesize{Ablation study of the trigger size.
We evaluate the bias scores with different trigger word numbers (\texttt{Civil Comments}) and different trigger size (\texttt{CelebA}) with fixed adversary weight $\lambda$.
}}

\label{fig: size_study}
\end{figure}

We perform an ablation study to investigate the effects of the trigger size.
Specifically, we run experiments with different numbers of trigger words / trigger patch sizes on the NLP / CV dataset.
We set a $\lambda$ value for each method such that all methods achieve comparable bias scores with the largest trigger size.
The detailed $\lambda$ choices can be seen in Appendix~\ref{app: training_detail}.
Then we train the triggers with different sizes in the tuning set using the fixed $\lambda$'s.  For the text trigger as shown in Fig.~\ref{fig: size_study}(a), we see that the negative bias score gets worse as the number of trigger words gets smaller.
However, our method can still improve fairness upon the \textsc{Base} model even with only a one-word trigger.
On the other hand, the results with five trigger words and above are all comparable, indicating that five words is enough to achieve the fairness goal.
Similarly, for the image trigger as shown in Fig.~\ref{fig: size_study}(b), the results suggest a larger trigger would consistently improve fairness.
On the other hand, we show that larger trigger size could hurt accuracy in Appendix~\ref{app: additional_results}, which is similar to the effect of increasing $\lambda$. 

\CR{\subsection{Summary of Additional Results}
We compare our proposed {\ours} with four additional baselines,
and we show the full results with variance in Tab.~\ref{tab: overview}. 
We further compare our method with MMD methods where $\mathcal{L}_{fair}$ in Eq.~\eqref{eq:loss} is replaced with Maximum Mean Discrepancy regularization~\cite{Louizos2016THEVF} to partial out the instability of adversarial training, and the results are shown in Fig.~\ref{fig: rebuttal_mmd}.
We also implement the fairness reprogramming in the black-box setting on \texttt{CelebA} dataset, where the model parameters are not available for training the reprogram, and the results are shown in Fig.~\ref{fig: blackbox}. 
Besides, we show that {\ours} could also be used in tabular data, and the corresponding experiment results on the \texttt{Adult} dataset are shown in Fig.~\ref{fig: rebuttal_tabular}.
}

==> ArXiv Fairness Reprogramming/relate.tex <==
\section{Related Work}

\paragraph{Fairness in ML}
Fairness problems in ML models have received increasing attention from both industry~\cite{Holstein2019ImprovingFI} and academia~\cite{Chouldechova2018TheFO,Sun2019MitigatingGB,Mehrabi2021ASO,Field2021ASO}.  
There has been a myriad of fairness definitions in the literature~\cite{Dwork2012FairnessTA,Chouldechova2018TheFO,Makhlouf2020SurveyOC,Hashimoto2018FairnessWD}.
Among them, group fairness notions are one of the most popular~\cite{Calders2010ThreeNB,Hardt2016EqualityOO,Rz2021GroupFI}, which require ML models to perform similarly for different demographic groups.   
In this paper, we mainly focus on the two most widely-used group fairness definitions, demographic parity~\cite{Calders2010ThreeNB} and equalized odds~\cite{Hardt2016EqualityOO}, but it is worth mentioning that our method is general for other fairness notions.  
Existing fairness promoting methods can be broadly categorized into pre-processing, in-processing, and post-processing methods~\cite{Caton2020FairnessIM}.  
Pre-processing methods calibrate the training data to remove the spurious correlations and train fair model on the modified data~\cite{Kamiran2011DataPT,Zemel2013LearningFR,Feldman2015CertifyingAR,Calmon2017OptimizedPF,Park2018ReducingGB,Dixon2018MeasuringAM,Grover2020FairGM,Zhang2020DemographicsSN}.  
In-processing methods work on training ML with extra fairness-aware regularization~\cite{Zafar2017FairnessCM,Agarwal2018ARA,Kamishima2012FairnessAwareCW,Baharlouei2019RenyiFI,PrezSuay2017FairKL,Roh2020FRTrainAM,Zhang2019FAHTAA}.  
For example, an adversarial framework is introduced to train model parameters to meet fairness requirements~\cite{Zhang2018MitigatingUB}.  
In our method, we adopt a similar adversarial loss but optimize the fairness triggers with a fixed model.
Despite the effectiveness, these methods usually consider training fair models from scratch and do not directly apply to already-trained models.  
Post-processing methods focus on calibrating trained ML models to be fair~\cite{Caton2020FairnessIM}.  
Many of them modify the model outputs to meet the fairness criteria~\cite{Dwork2012FairnessTA,Hardt2016EqualityOO,Petersen2021PostprocessingFI,Wei2020OptimizedST,Awasthi2020EqualizedOP,Woodworth2017LearningNP,Mishler2021FairnessIR,Zhao2017MenAL,Kim2019MultiaccuracyBP,Lohia2019BiasMP, Lohia2021PrioritybasedPB,Dwork2018DecoupledCF,Chzhen2019LeveragingLA}.  
For example,  the model outputs are directly modified to meet equalized odds by solving an optimization problem~\cite{Hardt2016EqualityOO}.  
Alternatively, a boosting-based method is introduced to calibrate model outputs \cite{Kim2019MultiaccuracyBP}.

\paragraph{Model reprogramming} 
Model reprogramming~\cite{bahng2022visual, tsai2020transfer, elsayed2018adversarial, neekhara2018adversarial, neekhara2022cross, zheng2021adversarial} aims to repurpose an already trained neural network for different tasks. 
Different from the typical transfer learning that requires modifying the structure and parameters of the given pre-trained model, reprogramming technology instead designs a trainable program appended to the input, while keeping the pre-trained model intact.  
The model reprogramming technology can be designed in the form of an input-agnostic perturbation~\cite{bahng2022visual, elsayed2018adversarial} or a trainable input transformation function together with the label mapping from the source domain to the target domain~\cite{tsai2020transfer}.
In particular, the feasibility of designing a universal input perturbation to reprogram a well-trained ImageNet classifier to the CIFAR-10 dataset is demonstrated in the white-box setting~\cite{elsayed2018adversarial}.  
As an exploration to implement reprogramming in the discrete scenario, another work~\cite{neekhara2018adversarial} successfully reprograms the text classification neural network for alternate classification tasks. 
This work also shows the possibility of developing reprogramming in the black-box setting, where the reprogrammer may not have the access to the parameters of the target model. 
Recent work~\cite{neekhara2022cross} shows the possibility of repurposing deep neural networks designed for image classifiers for the natural language processing and other sequence classification tasks.
It is argued the success of the reprogramming lies in the size of the average input gradient and the input dimension is crucial to the performance of the reprogrammer~\cite{zheng2021adversarial}. 
\CR{It is also shown that generative models like FairGANs~\cite{Xu2018FairGANFG} can be transfered to other tasks by reprogramming with variational auto-encoders~\cite{Nobile2022ReprogrammingFW}.}
A highly related topic to model reprograming is prompt learning in NLP~\cite{Ding2022OpenPromptAO}. 
It is shown that by designing designated text prompts appended to inputs, pre-trained language models could be re-directed to perform well under downstream tasks in a few-shot setting~\cite{Gao2021MakingPL}.
Prompt-based tuning methods have become the mainstream and achieve better performance than fine-tuning in many scenarios~\cite{Li2021PrefixTuningOC,Schick2021ItsNJ,Shin2020ElicitingKF,Diao2022BlackboxPL}. 
Seminal works
about prompt learning can be found in~\cite{Ding2022OpenPromptAO,Liu2021PretrainPA}.  
\textit{However},
nearly all existing methods focus on using model reprogramming to improve accuracy in domain-transfer tasks and to our best knowledge, our work is the first to generalize model reprogramming to improve fairness of a trained model.







==> ArXiv Fairness Reprogramming/theory.tex <==
It is not immediately straightforward why a \emph{global} trigger can obscure the demographic information for \emph{any} input. In this section, we will illustrate one of the mechanisms through which the trigger can remove the demographic information under a simplified setting. As we will show, if the trigger word is strongly indicative of a certain demographic group, then the the demographic information in $\hat{Y}$ will be obscured.

Consider a simple bag-of-word or bag-of-feature scenario, where
\begin{equation}
    \bm X = [\bm X_1, \bm X_2, \cdots, \bm X_T],
\end{equation}
Each $\bm X_i$ represents a word or a feature. For simplicity, we will refer to it as a word throughout this section. Note that $T$ can be variable. We further assume that the words in $\bm X$ can be divided into two groups,
\begin{equation}
    \bm X = [\bm X^y, \bm X^z],
\end{equation}
where $\bm X^y$, which we call \emph{output-related words}, constitutes the words whose probability distribution of $\bm X^y$ is governed by $Y$, and $\bm X^z$, which we call \emph{demographic-related words}, constitutes the words whose probability distribution is governed by $Z$. More specifically
\begin{equation}
    \quad p(\bm X^y | Y) = \prod_t p(\bm X^y_t | Y), \quad p(\bm X^z | Z) = \prod_t p(\bm X^z_t | Z).
\end{equation}
The probabilistic graph is shown in **. Note that although $\bm X^y$ is not directly indicative of $Z$, it may still be correlated with $Z$ because $Y$ and $Z$ may be spuriously correlated, and similarly for $\bm X^z$ and $Y$.

Each $\bm X^y_t$ is drawn from a vocabulary $\mathcal{X}^y$, and each $\bm X^z_t$ is drawn from a vocabulary $\mathcal{X}^z$. We assume that these two vocabulary sets are disjoint, \emph{i.e.} $\mathcal{X}^y \cap \mathcal{X}^z = \varnothing$. Assume that there is only one appended trigger word. If this trigger $\bm \delta$ is also a demographic-related word, \emph{i.e.} $\bm \delta \in \mathcal{X}^z$, then it should be absorbed into the $\bm X^z$ part. Formally, the perturbed input can be represented as
\begin{equation}
    \tilde{\bm X} = [\bm X^y, \tilde{\bm X}^z], \quad \mbox{where } \tilde{\bm X}^z = [\bm \delta, \bm X^z].
\end{equation}
In the following, we will be focusing on this scenario.

It can be shown that when inferring $Y$ from $\bm X$, $p_Z(\cdot |\bm X^z)$ is the sufficient statistics for $\bm X^z$ and $p_Y(\cdot | \bm X^y)$ is the sufficient statistics for $\bm X^y$ (we use $\cdot$ to denote the entire posterior distribution function). If the fixed classifier is unbiased, it should only depend on $p(Y | \bm X^y)$. Unfortunately, due to various reasons, an actual classifier may also refer to $p(Z|\bm X^z)$. Thus the classifier's output can be represented as
\begin{equation}
    \hat Y = f(p^{tr}_Y(\cdot | \bm X^y), p^{tr}_Z(\cdot|\bm X^z)).
    \label{eq:classifier}
\end{equation}
Note that we specially add a superscript $tr$ to emphasize that it is the training set distribution instead of the test distribution, because the classifier has never seen perturbed examples during training. Equation~\eqref{eq:classifier} encompasses a wide range of decision functions. For example, it can be shown that the posterior distribution of $Y$, $p(Y|\bm X)$, is a special case of Equation~\eqref{eq:classifier}.

Without loss of generality, consider the case where $Z$ is binary with uniform prior. Define the occurrence ratio $r(\bm \delta)$ as
\begin{equation}
    r(\bm \delta) = \frac{p^{tr}(\bm X^z = \bm \delta | Z = 1)}{p^{tr}(\bm X^z = \bm \delta | Z = 0)}.
\end{equation}
$r(\bm \delta)$ measures how much the value of $\bm \delta$ indicates each demographic group in the training set. If $r(\bm \delta)$ approaches 0, it is strongly indicative of demographic group 0. If $r(\bm \delta)$ approaches $+\infty$, it is strongly indicative of demographic group 1.

Now we are all set with the settings and ready to state of main conclusion.
\begin{theorem}
If $r(\bm \delta) \rightarrow 0$ or if $r(\bm \delta) \rightarrow +\infty$, then
\begin{equation}
    MI(Z, \hat{Y} | Y) \rightarrow 0,
\end{equation}
which means the equalized odds will hold. Further, if $\bm Z \perp Y$, then
\begin{equation}
    MI(Z, \hat{Y}) \rightarrow 0,
\end{equation}
which means demographic parity will also hold.
\end{theorem}

\begin{proof}
First, it can be shown by the Bayesian rule that when $r(\bm \delta) \rightarrow 0$, $p^{tr}_Z(0 | \tilde{\bm X}^Z) \rightarrow 1$; when $r(\bm \delta) \rightarrow 1$, $p^{tr}_Z(1 | \tilde{\bm X}^Z) \rightarrow 1$. In both cases, we have
\begin{equation}
    p^{tr}_Z(\cdot|\tilde{\bm X}^z) \rightarrow \bm c.
\end{equation}
where $\bm c$ is some constant. Therefore
\begin{equation}
    \hat Y = f(p^{tr}_Y(\cdot | \bm X^y), p^{tr}_Z(\cdot|\tilde{\bm X}^z)) \rightarrow f(p^{tr}_Y(\cdot | \bm X^y), \bm c)
\end{equation}
Note that the second term, which is the main source of the demographic information, gets obscured to a constant. Therefore, the demographic information will be removed in $\hat{Y}$. Formally,
\begin{equation}
\begin{aligned}
    H(Z | \hat{Y}, Y) &= H(Z | f(p^{tr}_Y(\cdot | \bm X^y), p^{tr}_Z(\cdot|\tilde{\bm X}^z)), Y) \\
    &\rightarrow H(Z | f(p^{tr}_Y(\cdot | \bm X^y), \bm c), Y) \\
    &\geq H(Z | p^{tr}_Y(\cdot | \bm X^y), Y) \\
    &\geq H(Z | \bm X^y, Y) \\
    &= H(Z | Y).
\end{aligned}
\label{eq:proof}
\end{equation}
Since $H(Z | \hat{Y}, Y) \leq H(Z | Y)$ always holds. Equation~\eqref{eq:proof} implies that
\begin{equation}
     H(Z | \hat{Y}, Y) \rightarrow H(Z | Y).
\end{equation}
\end{proof}

==> analysis.tex <==
\begin{table*}[t]
	\small
	\begin{tabular}{p{0.77\textwidth}c}
        \emph{Text (Non-toxic)} & \emph{Predicted Toxicity} \\
		\arrayrulecolor{grey}  
		\midrule
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlg{\ul{\textbf{the}}}{15} \hlr{\ul{\textbf{mirror}}}{20} & 0.149 \\
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlr{the}{0} \hlr{mirror}{0} \,\,\,\,
        \hlr{same}{0} \hlr{\ul{\textbf{diocesan}}}{15} \hlg{\ul{\textbf{bula}}}{20} \hlr{\ul{\textbf{rev}}}{8} \hlr{\ul{\textbf{proceedings}}}{8} & 0.069 \\
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlr{the}{0} \hlr{mirror}{0}  \,\,\,\,
        \hlr{soto}{0} \hlr{\ul{\textbf{cc}}}{10} \hlr{rib}{0} \hlr{\ul{\textbf{hebrew}}}{10} \hlr{armenian}{0} & 0.054 \\
        \hlg{\ul{\textbf{muslims}}}{20} \hlr{need}{0} \hlr{to}{0} \hlr{take}{0} \hlr{a}{0} \hlr{look}{0} \hlr{in}{0} \hlr{the}{0} \hlg{\ul{mirror}}{0}  \,\,\,\,
        \hlr{\ul{\textbf{paul}}}{10} \hlr{long}{0} \hlr{course}{0} \hlr{\ul{\textbf{parish}}}{10} \hlr{\ul{\textbf{body}}}{10} & 0.073 \\
	\end{tabular}
    \captionof{figure}{\small{
    A text example from \texttt{Civil Comments} with \textsc{Integrated Gradient}~\cite{Sundararajan2017AxiomaticAF,kokhlikyan2020captum}  highlighting important words that influence \textsc{ERM} model predictions.
    The text is concatenated with three triggers generated with different adversary weight.
    \hlg{\ul{\textbf{Green highlights}}}{20} the words that lean to toxic predictions and 
    \hlr{\ul{\textbf{Red highlights}}}{20} non-toxic leaning words.
    The model prediction tends to be correct after adding the triggers.
    }}
    \label{fig: vis_nlp}
    \vspace*{-4mm}
\end{table*}

\begin{wrapfigure}{r}{80mm}
    \vspace*{-4mm}
    \centering
    \includegraphics[width=\linewidth]{figures/grad_cam_small.png}
    \vspace*{-4.5mm}
    \caption{\footnotesize{Gradient-based saliency map visualized with \textsc{Grad Cam}~\cite{selvaraju2017grad} of different methods. 
    The highlighted zones (marked in red) depicting regions exerting major influence on the predicted labels (non-blond hair v.s. blond hair) in each row, which also depict the attention of the model on the input image.
    }}
    \label{fig: vis_cv}
    \vspace*{-1mm}
\end{wrapfigure}

\vspace*{-0.1in}
\paragraph{Input saliency attribution.}
Fig.~\ref{fig: vis_nlp} and \ref{fig: vis_cv} compare the saliency maps of some example inputs with and without the fairness triggers. Specifically, 
For the NLP applications, we extract a subset of \texttt{Civil Comments} with religion-related demographic annotations,
and apply IG~\cite{Sundararajan2017AxiomaticAF} to localize word pieces that contribute most to the text toxicity classification.  For the CV application, we use GradCam~\cite{selvaraju2017grad} to identify class-discriminative regions of   {\texttt{CelebA}}'s  test images.
As shown in Fig.~\ref{fig: vis_nlp}, our fairness trigger consists of a lot of religion-related words (\textit{e.g.}, diocesan, hebrew, parish). Meanwhile, the predicted toxicity score of the benign text starting from `muslims' significantly reduces. These observations verify our theoretical hypothesis that the fairness trigger is strongly indicative of a certain demographic group to prevent the classifier from using the true demographic information.
In addition, Fig.~\ref{fig: vis_cv} presents the input saliency maps on two input images with respect to their predicted labels, non-blond hair and blond hair, respectively. As can be observed, when there is no fairness trigger, the saliency region incorrectly concentrates on the facial parts, indicating the classifier is likely to use biased information, such as gender, for its decision. With the fairness trigger, the saliency region moves to the hair parts, which matches the behavior of \textsc{AdvIn}. These results confirm that our fairness trigger can drive models to make fairer predictions.



==> theory.tex <==
It is not immediately straightforward why a \emph{global} trigger can obscure the demographic information for \emph{any} input. In this section, we will illustrate one of the mechanisms through which the trigger can remove the demographic information under a simplified setting. As we will show, if the trigger word is strongly indicative of a certain demographic group, then the the demographic information in $\hat{Y}$ will be obscured.

Consider a simple bag-of-word or bag-of-feature scenario, where
\begin{equation}
    \bm X = [\bm X_1, \bm X_2, \cdots, \bm X_T],
\end{equation}
Each $\bm X_i$ represents a word or a feature. For simplicity, we will refer to it as a word throughout this section. Note that $T$ can be variable. We further assume that the words in $\bm X$ can be divided into two groups,
\begin{equation}
    \bm X = [\bm X^y, \bm X^z],
\end{equation}
where $\bm X^y$, which we call \emph{output-related words}, constitutes the words whose probability distribution of $\bm X^y$ is governed by $Y$, and $\bm X^z$, which we call \emph{demographic-related words}, constitutes the words whose probability distribution is governed by $Z$. More specifically
\begin{equation}
    \quad p(\bm X^y | Y) = \prod_t p(\bm X^y_t | Y), \quad p(\bm X^z | Z) = \prod_t p(\bm X^z_t | Z).
\end{equation}
The probabilistic graph is shown in **. Note that although $\bm X^y$ is not directly indicative of $Z$, it may still be correlated with $Z$ because $Y$ and $Z$ may be spuriously correlated, and similarly for $\bm X^z$ and $Y$.

Each $\bm X^y_t$ is drawn from a vocabulary $\mathcal{X}^y$, and each $\bm X^z_t$ is drawn from a vocabulary $\mathcal{X}^z$. We assume that these two vocabulary sets are disjoint, \emph{i.e.} $\mathcal{X}^y \cap \mathcal{X}^z = \varnothing$. Assume that there is only one appended trigger word. If this trigger $\bm \delta$ is also a demographic-related word, \emph{i.e.} $\bm \delta \in \mathcal{X}^z$, then it should be absorbed into the $\bm X^z$ part. Formally, the perturbed input can be represented as
\begin{equation}
    \tilde{\bm X} = [\bm X^y, \tilde{\bm X}^z], \quad \mbox{where } \tilde{\bm X}^z = [\bm \delta, \bm X^z].
\end{equation}
In the following, we will be focusing on this scenario.

It can be shown that when inferring $Y$ from $\bm X$, $p_Z(\cdot |\bm X^z)$ is the sufficient statistics for $\bm X^z$ and $p_Y(\cdot | \bm X^y)$ is the sufficient statistics for $\bm X^y$ (we use $\cdot$ to denote the entire posterior distribution function). If the fixed classifier is unbiased, it should only depend on $p(Y | \bm X^y)$. Unfortunately, due to various reasons, an actual classifier may also refer to $p(Z|\bm X^z)$. Thus the classifier's output can be represented as
\begin{equation}
    \hat Y = f(p^{tr}_Y(\cdot | \bm X^y), p^{tr}_Z(\cdot|\bm X^z)).
    \label{eq:classifier}
\end{equation}
Note that we specially add a superscript $tr$ to emphasize that it is the training set distribution instead of the test distribution, because the classifier has never seen perturbed examples during training. Equation~\eqref{eq:classifier} encompasses a wide range of decision functions. For example, it can be shown that the posterior distribution of $Y$, $p(Y|\bm X)$, is a special case of Equation~\eqref{eq:classifier}.

Without loss of generality, consider the case where $Z$ is binary with uniform prior. Define the occurrence ratio $r(\bm \delta)$ as
\begin{equation}
    r(\bm \delta) = \frac{p^{tr}(\bm X^z = \bm \delta | Z = 1)}{p^{tr}(\bm X^z = \bm \delta | Z = 0)}.
\end{equation}
$r(\bm \delta)$ measures how much the value of $\bm \delta$ indicates each demographic group in the training set. If $r(\bm \delta)$ approaches 0, it is strongly indicative of demographic group 0. If $r(\bm \delta)$ approaches $+\infty$, it is strongly indicative of demographic group 1.

Now we are all set with the settings and ready to state of main conclusion.
\begin{theorem}
If $r(\bm \delta) \rightarrow 0$ or if $r(\bm \delta) \rightarrow +\infty$, then
\begin{equation}
    MI(Z, \hat{Y} | Y) \rightarrow 0,
\end{equation}
which means the equalized odds will hold. Further, if $\bm Z \perp Y$, then
\begin{equation}
    MI(Z, \hat{Y}) \rightarrow 0,
\end{equation}
which means demographic parity will also hold.
\end{theorem}

\begin{proof}
First, it can be shown by the Bayesian rule that when $r(\bm \delta) \rightarrow 0$, $p^{tr}_Z(0 | \tilde{\bm X}^Z) \rightarrow 1$; when $r(\bm \delta) \rightarrow 1$, $p^{tr}_Z(1 | \tilde{\bm X}^Z) \rightarrow 1$. In both cases, we have
\begin{equation}
    p^{tr}_Z(\cdot|\tilde{\bm X}^z) \rightarrow \bm c.
\end{equation}
where $\bm c$ is some constant. Therefore
\begin{equation}
    \hat Y = f(p^{tr}_Y(\cdot | \bm X^y), p^{tr}_Z(\cdot|\tilde{\bm X}^z)) \rightarrow f(p^{tr}_Y(\cdot | \bm X^y), \bm c)
\end{equation}
Note that the second term, which is the main source of the demographic information, gets obscured to a constant. Therefore, the demographic information will be removed in $\hat{Y}$. Formally,
\begin{equation}
\begin{aligned}
    H(Z | \hat{Y}, Y) &= H(Z | f(p^{tr}_Y(\cdot | \bm X^y), p^{tr}_Z(\cdot|\tilde{\bm X}^z)), Y) \\
    &\rightarrow H(Z | f(p^{tr}_Y(\cdot | \bm X^y), \bm c), Y) \\
    &\geq H(Z | p^{tr}_Y(\cdot | \bm X^y), Y) \\
    &\geq H(Z | \bm X^y, Y) \\
    &= H(Z | Y).
\end{aligned}
\label{eq:proof}
\end{equation}
Since $H(Z | \hat{Y}, Y) \leq H(Z | Y)$ always holds. Equation~\eqref{eq:proof} implies that
\begin{equation}
     H(Z | \hat{Y}, Y) \rightarrow H(Z | Y).
\end{equation}
\end{proof}
